Exploring the effects of robotic design on learning and neural control

The ongoing deep learning revolution has allowed computers to outclass humans in various games and perceive features imperceptible to humans during classification tasks. Current machine learning techniques have clearly distinguished themselves in specialized tasks. However, we have yet to see robots capable of performing multiple tasks at an expert level. Most work in this field is focused on the development of more sophisticated learning algorithms for a robot's controller given a largely static and presupposed robotic design. By focusing on the development of robotic bodies, rather than neural controllers, I have discovered that robots can be designed such that they overcome many of the current pitfalls encountered by neural controllers in multitask settings. Through this discovery, I also present novel metrics to explicitly measure the learning ability of a robotic design and its resistance to common problems such as catastrophic interference. Traditionally, the physical robot design requires human engineers to plan every aspect of the system, which is expensive and often relies on human intuition. In contrast, within the field of evolutionary robotics, evolutionary algorithms are used to automatically create optimized designs, however, such designs are often still limited in their ability to perform in a multitask setting. The metrics created and presented here give a novel path to automated design that allow evolved robots to synergize with their controller to improve the computational efficiency of their learning while overcoming catastrophic interference. Overall, this dissertation intimates the ability to automatically design robots that are more general purpose than current robots and that can perform various tasks while requiring less computation.

==> proposed.tex <==
\section{Summary of Current Work}
My initial work in the area of catastrophic interference compared robots with identical neural controllers and sensors. Each robot differed in their design as described in chapter 2 of this proposal. This work mainly showed that the robots body plan had a distinctive effect on the ability of the neural controller to resist catastrophic interference. One of the robot designs even allowed it to completely overcome the problem. However, this work did not examine any effects on the speed of learning or in other words their computational efficiency. Furthermore, it did not give any details into how or why the specific robot design allowed the neural controller to overcome this problem.

The next stage of my work, described in chapter 3 of this proposal, examined the optimial parameters space of neural controllers over variations in the sensor placement in a simple robot. This research explains how robot design changes the optimal parameters space and thus allow certain designs to overcome catastrophic interference. It further postulated that robots with designs resistant to catastrophic interference would likely have an increased learning rate as well. However, the results of this research were mainly theoretical and not experimentally validated.

The proposed work would serve two main purposes, first to validate the theoretical work of from chapter 3 in an experimental setting, and second to give an explanation as to why the designs described actually change the optimal parameters space in this manner. Doing both of these would allow myself and others to augment the field of automated design by allowing for the creation of robots that are robust, learn quickly, and perform well in multitask settings.

\section{Validating Theory with Experiments}
In chapter three of this proposal, I introduced two metrics to measure a robot's resistance to catastrophic interference ($M_{CF}$ see ~\ref{eq:metric2}) and to measure it's learnability ($M_L$ see ~\ref{eq:metric1}). However, as stated, the measurements were not then validated with experimental results. Thus, I propose to perform that validation. I will also extend the scope of the research to include a metric to test whether certain morphologies may also result in a reduced need for complexity.

\subsection{The Neural Controllers}
To augment the previous work, I would expand the 2 dimensional neural controller used in the study to include high dimensional neural networks and architectures commonly used in robotics research. However, since it will be infeasible to do a comprehensive sweep over the optimizable parameters for higher dimensional networks, I will test each neural network on every robot design across a variety of training methods. This will validate that the findings in chapter two actually result in a reduction of catastrophic interference and improved training times.

The extension of this research will also test whether certain morphologies reduce the need for complex controllers. This requires a structured enumeration of neural networks that grow in both size and complexity. I will start this enumeration with the most basic of neural networks---a fully connected network from the input sensors to the output motors---and expand both the number of neurons and the number of hidden layers as shown in Fig.~\ref{fig:enumeration}.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/enum.png}
    \caption{A visual description of an enumeration pattern for increasing both the size of a neural network (i.e. total number of trainable parameters) and the number of hidden layers of the network (i.e. complexity) that has two inputs and two outputs.}
    \label{fig:enumeration}
\end{figure}

I will then compare each design to that of the design with the standard sensor placement just as in the original study. I will measure whether any of these nonstandard designs reach or exceed the the performance of the standard design while requiring a smaller neural network and/or less complex one.


\subsection{Training Algorithms}
In a similar fashion to the sweep over various designs and neural architectures I plan to sweep through a variety of training algorithms that will include the most popular evolutionary optimizers \cite{hansen2020coco}, and the most popular optimizers in deep reinforcement learning \cite{pmlr-v48-duan16} that do not directly address catastrophic interference.

\subsection{Potential Results}
The measurement of results and determination of success is described by Fig.~\ref{fig:corrl}, and includes a series of analysis. The first is that a higher learnability metric for a design should correlate with reduced training time across training methods. Similarly, a high score on resistance to catastrophic forgetting should correlate with higher levels of attained fitness. If both of these criteria are met then the theoretical results of the previous work would indeed be indicative of real world performance. Additionally, we want to know if these metrics correlate with reduced complexity. This analysis would explore whether either or both of the previously defined metrics are correlated with reduced differences between the performance of different network architectures.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/plot_L.png}
    \includegraphics[width=0.45\textwidth]{Figures/plot_MC.png}
    \includegraphics[width=0.45\textwidth]{Figures/plot_Comp.png}
    \caption{(TL) A higher learnability score $M_L$ should correlate with reduced training times. (TR) A higher resistance to catastrophic interference $M_{CF}$ should correlate with better multitask performance. (BM) There should be no correlation between complexity and performance for a design with a high score on both metrics.}
    \label{fig:corrl}
\end{figure}

\section{Why does design change the optimal parameter space}
The previous section of this proposal mainly deals with how the optimal parameter space changes in response to different designs. The last section of this proposal is an attempt to explain at least one reason why some designs change the optimal parameter space in such a favorable manner. I propose to do this by building on the work described in chapter two of this document. In that chapter I compared three quadruped robots with different designs (one has only legs, one only wheels, and one, a combination of legs and wheels). However, each of the robots has the same sensor inputs and number of motor outputs and thus equal neural architectures. In that work I found that one of the robot designs was able to consistently overcome catastrophic interference. In visual analysis of this robot's behavior we found that it moved almost identically in the differing environments, while the other designs had different behaviors for each new location of the light source. I postulated in the discussion that perhaps the one design allowed for a condensing of the environments such that the different environments appear very similar to each other. This would be equivalent to creating a large overlap between the various optimal parameter spaces as discussed in chapter three. I propose an analysis (via the dynamic time warping algorithm) of the sensor input data of these robots to determine if in fact the environments are condensed into one from the robots point of view.

\subsection{Dynamic Time Warping}
Dynamic time warping (DTW) \cite{muller2007dynamic} is an algorithm that measures the similarity between two temporal sequences. As an example, DTW could be used to score the similarities between walking gaits, accounting for differences in speed or acceleration. It has also been applied to sequences of video and audio data, and in general can be used for any linear sequence. I propose to use this algorithm to analyze the similarity between robot sensor data of one design in differing the differing environments (light source locations). If the signal between different environments in the best design is significantly more similar than the other designs, this shows that the robot sees the environments as the same; thus serving as an explanation as to why a particular design creates and overlaps between optimal parameter spaces.

\subsection{Homeostasis as a fitness objective}
The principle of keeping your internal environment the same in the face of external changes is known as homeostasis. Biology is filled with examples of animals that adapt to maintain homeostasis. A simple example would be a human that puts on a coat in cold weather to maintain a constant sensory temperature on their skin. All previous designs in this proposal were found by a sweep over many possible designs or were found by chance. I would like to incorporate homeostasis as a guiding principles in the automatic design of robots as a method for developing more efficient-multi-task robots. To do this, I propose a final method that incorporates DTW as a fitness objective in the evolution of a robot design. I will compare this design to the three previous hand designs to test the effectiveness of this strategy. Thus, this final section of the proposal will provide a concrete example and direction for using design as a method to overcome catastrophic interference in the field of robotics.

\section{Conclusion}
Overall, the goal of this research is three fold. First, to determine how a robot design impacts the optimal parameters space of a robot in a multi-task setting such that it may overcome current pitfalls in the training of neural networks. Second, to determine why certain robot designs have effects on the optimal parameter space that cause them to overcome catastrophic interference. Third, to find additional design principles that can guide the automatic optimization of robot design. Ultimately, this research would contribute to multiple fields including neural networks, evolutionary robotics, and automated design. My approach uses novel methods to explore problems in these areas and lays the groundwork for future research in these domains.


